Towards Translating Real-World Code with LLMs: A Study of Translating to Rust

Large language models (LLMs) show promise in code translation - the task of translating code written in one programming language to another language - due to their ability to write code in most programming languages. However, LLM's effectiveness on translating real-world code remains largely unstudied. In this work, we perform the first substantial study on LLM-based translation to Rust by assessing the ability of five state-of-the-art LLMs, GPT4, Claude 3, Claude 2.1, Gemini Pro, and Mixtral. We conduct our study on code extracted from real-world open source projects. To enable our study, we develop FLOURINE, an end-to-end code translation tool that uses differential fuzzing to check if a Rust translation is I/O equivalent to the original source program, eliminating the need for pre-existing test cases. As part of our investigation, we assess both the LLM's ability to produce an initially successful translation, as well as their capacity to fix a previously generated buggy one. If the original and the translated programs are not I/O equivalent, we apply a set of automated feedback strategies, including feedback to the LLM with counterexamples. Our results show that the most successful LLM can translate 47% of our benchmarks, and also provides insights into next steps for improvements.

==> aux.tex <==
\cd{
Program transpilation is concerned with translating  source code written in one language to another language, with a similar level of abstraction. This task is becoming particularly relevant, given the recent interest in new, safe programming languages such as Rust, and, the expectation of translating potentially buggy, legacy code into such modern languages.

At the same time, the promise of large, generalist language models (simply “LLMs” in this work), such as ChatGPT, provides the hope that transpilation can be done automatically by the LLMs. Unfortunately, a recent work casts doubt on this belief.  In particular, the robust study conducted in \cite{PanICSE24} revealed that LLMs can't be reliably used to automate code translation, with correct translations ranging from 2.1\% to 47.3\% for the studied LLMs. Even worse, the study concluded that the LLMs were largely ineffective on real-world projects, with success rates of 8.1\% for GPT-4 and 0\% for the rest of the models. As a 
way of improving the performance of the LLMs, the authors of \cite{PanICSE24}  propose an iterative prompting approach that incorporates additional information about the failure (e.g. previous unsuccessful translation, stack trace, error messages from failing execution, failing test cases), which they found it increases the success rate by 5.5\%, on average.

In the current work, we revisit and challenge some of the conclusions of this recent study. In particular, our focus is on investigating the efficacy of a number of fallback strategies applied whenever the LLM provides an incorrect answer to a translation task:
\begin{enumerate}
    \item restart by throwing away the code candidate and generating a new query,
    \item repair by providing information about the error the code candidate using the counterexample,
    \item respond by building a back-and-forth dialogue with the LLM, and
    \item parameter search by automatically tuning model parameters, e.g. temperature.
\end{enumerate}

Our conclusion is that the conventional wisdom (perpetuated by \cite{PanICSE24} ) that providing more information to the LLM might not hold true for translation tasks. Instead, we showcase the advantage of other fallback/recovery techniques, such as restarts. \textbf{[here we need some numbers]}

The particular transpilation problem we address in this paper is that of going from C and Go to Rust. We picked  C and Go as source languages due to their different memory management protocols, with the former being manually managed, and the latter using a garbage collector. Memory management plays a central role in Rust, and finding the correct mapping between source and target is particularly difficult, even when done manually by experienced programmers. Considering different memory management protocols for the source language increases the confidence in the results of the study, as well as their transferability to other languages.

In order to make the problem more challenging, and avoid contaminating the study's results, we exclude the handling of Rust compilation errors from the study. The reason for this decision is the fact that the Rust compiler provides comprehensive error messages (containing clear suggestions for fixing the errors), which result in a much higher repair rate for the LLM than for other errors. (We handle these errors separately with a success rate of ...\%).

We are considering real-world benchmarks.
}

==> data_availability.tex <==
\section{Data Availability}
We open source all code, benchmarks, results to reproduce our experiments at \url{https://d34gtk3knhjgeg.cloudfront.net/artifact.tar.gz}


==> intro5.tex <==
\section{Introduction}
\label{section:intro}


% motivate the use LLMs in code translation
% Recent work~\cite{} has shown that large, generalist language models (simply ``LLMs'' in this work), such as ChatGPT, are highly effective for program transpilation -- the task of translating a program from a source language to a different target language. 
%
% They are particular well-suited to the task because they work out-of-the-box on most programming languages without fine-tuning. Moreover, they are highly adaptable. For example, they can learn to use new tools and libraries by pasting documentation directly into the prompt~\cite{zeroshottoolusage}.
%
% However, LLMs still may generate incorrect translations that do not faithfully preserve the behavior of the original source program, and due to the stochastic techniques employed in LLM inference, this issue is unlikely to ever be resolved.

The task of program translation between programming languages is becoming particularly relevant, given the recent interest in safe programming languages such as Rust, and the expectation of translating potentially buggy, legacy code into such modern languages. While ``rule-based'' translation tools have been developed~\cite{cgo, sharpen,c2rust} that target a fixed source and target language (e.g. C to Rust), recent work~\cite{tang-etal-2023-explain, RoziereLachaux2020, RoziereZhang2022, szafraniec2022code} provides hope that large language models (LLMs) can accomplish this task for any source and target language.

% However, prior work in LLM-based transpilation has been limited at least in part due to the lack of tooling of automatically evaluating the (semantic) correctness of the translations.
Prior work in using LLMs for code translation~\cite{PanICSE24, tang-etal-2023-explain, RoziereLachaux2020, RoziereZhang2022, szafraniec2022code,jana2023attention} has almost exclusively focused on translating code taken from competitive programming websites~\cite{puri2021codenet}, educational websites~\cite{ahmad2021avatar}, or hand-crafted coding problems~\cite{liu2024your,chen2021evaluating}.
While useful, such benchmarks are not representative of real-world code. 
For example, these benchmarks are typically a single function using only primitive data types, whereas real-world code has many functions and user-defined data types (e.g. structs).

In this work, we take a step towards answering the question: Can LLM's translate real-world code?
Towards this end, we develop \tool{}, an end-to-end code translation tool capable of producing validated Rust translations.
\tool{} first uses an LLM to obtain a candidate translation, then applies a compilation driven repair, where we make use of the Rust compiler's error messages as described in \cite{deligiannis2023fixing}. Once the translation compiles, \tool{}
uses cross-language differential fuzzing to test the I/O equivalence between the source program and the Rust translation.
Notably, our cross-language differential fuzzer allows us to evaluate equivalence when unit tests are not present -- prior work assumed test cases already exist in the target language, or they were hand-written as part of the study, making a substantial investigation difficult. 
If a counterexample is discovered, \tool{} executes a \textit{feedback strategy}, which provides feedback to the LLM to fix the counterexample.


For the dataset we extract benchmarks from seven open source projects written in C and Go. We do not use the entire projects because LLMs cannot fit them in their context window.
We choose these languages because Rust, C, and Go are typically used for low-level programming tasks, such as systems development, so C and Go are likely candidates for translation to Rust.
The open source projects are from a diverse set of domains: audio processing, text processing, geometry, banking, 2D triangulation, graph algorithms, and sound card emulation.
To automate and reduce bias in the selection of code samples, we develop a methodology and tool for extracting them from projects.
We use this tool to extract code samples that contain between 1 and 25 functions and use only standard libraries, and which also use features such as global variables, user-defined, dynamically-allocated, data structures, array pointers, type casts, enumeration types etc..

%\cd{the fig doesn't contain the ids mentioned in the text}
%The high-level flow of \tool{} is shown in Figure~\ref{fig:overview}. \tool{}'s inputs are a source program $p$, which may have many functions and user-defined data types, with an entry point function $f$ (which doesn't have to be the \texttt{main} function). \tool{} outputs a new program $p'$ in the target language that has an entry point function $f'$, where $f$ and $f'$ are I/O equivalent. Internally, \tool{} first uses an LLM to produce a candidate translation, for which it applies compilation driven repair to obtain the compilable candidate translation $p'$. \tool{} then performs differential fuzzing between the entry points of $p$ and $p'$ to test their I/O equivalence. If a counterexample is found, a feedback strategy is invoked, which produces a new prompt to the LLM that generates a new translation candidate. This process is repeated until the candidate passes differential fuzzing, or fails after a fixed number of iterations is reached.

%Since $f$ (the source program's entry point) and $f'$ (the Rust program's entry point) are in two different languages, and their inputs and outputs may use pointers and user-defined types, we have two engineering challenges to solve.
%First, to leverage off-the-shelf fuzzing tools, $f$ and $f'$ must be executed in the same process. To solve this, we build our differential fuzzer in Rust, allowing us to natively invoke $f'$, and we invoke $f$ using a foreign function interface.
%Second, since our fuzzer generates inputs using Rust data types, we must be able to map those data types to the types used by $f$.
%To solve this, we develop a solution based on common serialization formats allowing us to pass inputs and outputs between languages.

\input{examples}


We evaluate the LLM's ability to produce compilable translations, as well as translations that preserve the source behavior.
Given that semantic equivalence is critical to program translation, we further investigate the LLM’s potential to take feedback and fix equivalence errors.
We develop and compare four different feedback strategies.
Three of our feedback strategies provide the the LLM with counterexamples returned by the fuzzer. We compare these with a baseline strategy that repeats the original prompt, relying on randomness in LLM inference to obtain a new candidate translation.

%\begin{figure}[t!]
%    \centering
%    \includegraphics[scale=0.45]
%    {figures/overview2.pdf}
%    \caption{High-level flow \tool{}.}
%    \label{fig:overview}
%\end{figure}

In total, we perform 8160 code translation experiments across 408 code samples, four feedback strategies and five state-of-the-art LLMs -- GPT4, Claude 3, Claude 2.1, Gemini Pro, and Mixtral.
Overall, the LLMs achieve successful translation rates of 21\% to 47\% on our code samples, and feedback strategies are responsible for up to 8\% absolute of this success rate.
Somewhat unsurprisingly, 
% open source LLMs still under-perform compared to proprietary LLMs, and 
we find that larger programs (in LoC) are less likely to translate successfully than smaller programs.
Surprisingly, we also find that our feedback strategies that include counterexamples in the prompt actually \textit{perform worse} than the simple baseline strategy. 
We discuss why this may be case, and suggest directions for future work.

We claim the following contributions:
\begin{itemize}
    \item We develop \tool{}, a tool capable of producing validated Rust translations without the need for hand-written test cases 
    \item We build a cross-language fuzzer, capable of passing inputs and outputs between languages
    \item We use \tool{} to conduct the first 
    %large-scale 
    substantial study of using LLMs to translate real-world code
    \item We demonstrate that LLMs are capable of translating parts of real-world projects, and that directly providing counterexamples as feedback to an LLM is less effective than repeating the original prompt
    \item We open source all code, benchmarks, results to reproduce our experiments\footnote{Artifact can be downloaded at \url{https://d34gtk3knhjgeg.cloudfront.net/artifact.tar.gz}} 
\end{itemize}



==> old/abstract.tex <==
\begin{abstract}
% Recently, there has been great interest in using LLMs for various code generation tasks such code completion, code generation from description and code translation from one language to another or simply transpilation. Main concern with using LLMs for code generation lies in lack of correctness guarantees. However, even at the presence of oracles that can decide whether the generation is passing relevant checks or not, it hasn't been structurized what actions to take, if the latter is the case. In this work, we aim to provide a general answer to what to do when the generated code fails some checks. For this, we analyze a wide range of fallback methods to understand how to utilize LLMs further in such cases. Given recent interest in Rust programming language, we consider a Rust transpilation case where we utilize LLMs for generating Rust code which is supposedly be semantically equal to the input code in another language. For checking their equivalence, we develop a cross-language fuzzing platform. For any non-passing program, we launch a fallback process which can be simple repeat which leverages non-determinism of LLM responses, model parameter search, task simplification, morphological prompt mutations and evidence based fix attempts. We also go one step further for fix process and present novel approaches for cleaning compilation and semantical errors. We assess effectiveness of each of these methods on $>$400 single file C and Go programs that are collected from real world open-source projects. We find out...
%
\if 0
LLMs hold promise in code translation -- the task of translating code in programming language to another -- due to their adaptable nature, but recent work suggests that LLMs often produce translations whose input-output behavior differs from the original source program.
%
Even if we know the buggy input and the expected output for a translation, a critical question remains unanswered: given a buggy translation and an input that exercises the bug, how can we effectively provide feedback to the LLM to fix the translation?
%
% We refer to techniques for providing this feedback as \textit{fallback methods}.
%
In this work, we aim to answer this question.
%
We first propose a comprehensive set of techniques that leverage the provided buggy inputs and expected outputs to provide feedback to an LLM. 
%
We refer to these techniques as \textit{fallback methods}.
%
To facilitate evaluating our fallback methods, we develop the first code translation tool that connects an LLM with an \textit{oracle} routine capable of validating the correctness of the LLM's translation.
%
Our oracle routine performs cross-language differential fuzzing to discover inputs where the translation and original source program differ.
%
When buggy inputs are discovered, a fallback method is then invoked to provide feedback to the LLM and generate a new translation.
%
Motivated by recent interest in translating code to Rust, we target translating C and Go code to Rust.
%
We also take a significant step forward in assessing the practicality of such an approach on real-world code.
%
We perform translation on a large number of benchmarks extracted from open source projects on Github. The benchmarks have multiple functions and use complex data types, unlike prior work.
%
In total, we gather XXX C and Go benchmarks, we propose seven different fallback methods, and we evaluate our fallback methods using three different state-of-the-art LLMs.
%
Our findings indicate that (1) counterexamples alone can be leveraged to great effect in guiding an LLM to fix an incorrect translation, and (2) LLMs are significantly more capable at translating real-world code than reported in prior work.
\fi
\if 0
% We present and evaluate the first oracle guided framework for using LLMs to generate and regenerate code. This framework includes a cross-language fuzzing platform, so the oracles can be implemented in different languages than the generation target. When code fails fuzzing, our framework provides a range of fallback strategies that use the oracle feedback to prompt the LLM for code regeneration. We perform a comprehensive analysis of these feedback strategies and find that the most successful strategy is our novel approach for breaking the original task into sub-tasks for the new prompt. We also describe cases where other approaches are more likely to succeed.

% We perform our evaluation on transpilation to Rust. The goal of this transpilation is to use LLMs to generate target Rust code that is semantically equivalent to input code from another language. We apply our framework to more than 500 C and Go programs extracted from real-world open-source projects. Those programs consists of multiple functions taking complex arguments, presenting a significantly higher level of complexity compared to the previously studied solutions to competitive programming problems.





%Recently, there has been a significant interest regarding the application of Language Models (LLMs) for diverse code generation tasks, such as code completion, code generation from descriptions, and transpilation—the process of translating code from one language to another. A primary concern associated with utilizing LLMs for code generation revolves around the absence of correctness guarantees. Even when oracles are present to determine whether the generated code meets relevant checks, a structured framework defining actions in case of failure is lacking. This work aims to address the overarching question of \emph{how to respond when generated code fails certain checks}. To achieve this, we undertake a comprehensive analysis of various fallback methods, seeking to enhance the utilization of LLMs in such scenarios. Inspired by the growing interest in the Rust programming language, we explore a Rust transpilation case where LLMs are employed to generate Rust code intended to be semantically equivalent to input code in another language. To assess their equivalence, we introduce a cross-language fuzzing platform. In instances where a program does not pass the required checks, we initiate a novel fallback process guided by worthhwhile observations.
% This process includes simple repetition leveraging the non-determinism of LLM responses, model parameter (e.g. \emph{temperature}) search, task simplification, morphological prompt mutations, and evidence-based fix attempts.  
% We provide valuable insights and a concrete recipe describing which method is more appropriate for which cases. Taking a step further in the fix process, we present novel approaches and worthwhile observations for addressing compilation and semantic errors effectively. 
%The effectiveness of our approach is evaluated on a dataset comprising more than 500 C and Go programs extracted from real-world open-source projects. Those programs consists of multiple functions taking complex arguments, presenting a significantly higher level of complexity compared to the previously studied solutions to competitive programming problems. Our findings show that...
\fi
%
LLMs hold promise in code transpilation---the task of translating software in one programming language to another---but way too often, even state-of-the-art LLMs produce translations that are wrong. In particular, LLMs are impractical when applied to industrial program transpilation tasks. We investigate how to fix the translation by guiding the LLM towards a correct answer. We connect the LLM to an oracle to determine whether the translated program is I/O equivalent to the original source program, and if not, apply a diverse set of automated feedback algorithms, including feedback to the LLM with counterexamples and a problem partitioning method. We quantify the benefit of our feedback by comparing to the LLM's initial response. On a set of software applications representative for industrial transpilation work, we observe that our conversational guidance improves the translation success rate from 23.3\% to 40.7\%. Our key insight is that breaking up large tasks into smaller sub-problems for the LLM outperforms any other feedback method.
\end{abstract}

\begin{IEEEkeywords}
LLMs, code transpilation, correctness
\end{IEEEkeywords}


==> old/intro.tex <==
\section{Introduction}
\label{section:intro}

% motivate the use LLMs in code generation, and tasks with oracles
Large, generalist language models (simply ``LLMs'' in this work), such as ChatGPT are highly adaptable for code generation. 
%
LLMs work on most programming languages out-of-the-box, they can work on many unseen tasks (i.e. zero-shot learning)~\cite{kojima2022large}, and they can learn to use new tools and libraries by pasting documentation directly into the prompt~\cite{hsieh2023tool}.

% motivate the study of llm-based code generation with input-output oracles
However, most prior work in LLM-based code generation does not consider the presence of an input-output \textit{oracle}, which is unfortunate because many code generation tasks have an oracle available that can be exploited.
%
For example, in code translation -- the task of rewriting a program in one language to another -- the original program serves as an oracle. 
%
In automated program repair (APR) -- the task of generating a patch for a buggy program -- we may have a set of test cases taking the form of input-output examples.
%
In some tasks, we may even have a formal input-output specification which the generated code can be verified against~\cite{clarkbarretdafnyllmpaper}.

{\color{blue} 
\textbf{Could something like below be used to link the idea of oracles and that of fallback strategies? (it is rough for now, but I can improve it, if you think it's worth it.)}

However, the role of such oracles for LLM-based code generation is surprisingly limited. When it comes to training, models generally use a next token prediction objective which maximizes the likelihood of the next ground truth token, thus completely ignoring the oracle [add citations]. This has been addressed in the literature by using reinforcement learning during training, where the reward signal considers the oracle.

At inference, oracles are sometimes used to provide correctness guarantees about the generated programs: a program that is validated by the oracle will behave as expected. However, we are still left with the question of how to proceed if the oracle deems the program as incorrect. While existing works attempt some ad-hoc repair (potentially based on counterexamples provided by the oracle [add citation]), there is no systematic investigation of oracle-guided fallback strategies for LLM-based code generation.   

To the best of our knowledge, this work is the first to develop and evaluate a LLM-based code translation pipeline that systematically investigates oracle-guided fallback strategies.}



% introduce the problem of correcting mistakes, define "fallback method", and go over the flow of the figure
The following question remains unanswered in the literature: when an LLM generates code whose actual output disagrees with the expected output of the oracle, what techniques are effective for providing feedback to the LLM to fix/resolve the disagreement?
%
We refer to such techniques as \textit{fallback methods}.
%
Figure~\ref{fig:overview} illustrates how fallback methods are used in code generation with oracles.
%
As shown in the figure, a description of a code generation task is first given to an LLM, which generates a code candidate. 
%
The candidate is checked against an oracle, which may provide a counterexample containing a program input, the expected output of the oracle, and the actual output of the code candidate.
%
If a counterexample is found, a fallback method is invoked, which uses the counterexample, generated code, and the original task to construct a new query to the LLM.
%
A new code candidate is generated with the new query, and this process repeats until the oracle does not return a counterexample.


A comprehensive study of fallback methods would benefit many code generation tasks, but such a study is lacking. 
%
Most prior work on LLM-based code generation~\cite{singlegencodegenworks,progsynthwLLMs}, automated program repair~\cite{singlegenerationAPRworks}, and code translation~\cite{singlegenerationCodeTranslationworks} do not consider the presence of an oracle during generation.
%
% They typically use the LLM to generate many code candidates, rank them, and then output the highest ranked candidate, but if the final code , they simply fail without attempting to remediate the disagreement.
%
% They focus on \textit{heuristic} based techniques for assessing the likelihood generated code is correct, such as developing \textit{ranking}\footnote{These ranking functions provide a probability that code is correct, which is not to be confused with ranking functions for loop invariants} functions, or self-consistency/introspection techniques which use an LLM to inspect, explain, and then possibly correct the generated code.
%
% Single-generation techniques are orthogonal to ours.
%
Only very recent works have considered the presence of an oracle~\cite{APRandTranslationworks}, however the fallback methods they consider are limited.
%
They either repeat the same query to get a new code candidate, or they provide the failing input and the correct output as response to the LLM and ask the LLM to fix it.

% - TODO: mention program synthesis from examples and/or specifications
% - TODO: clarify that compilers as oracles is not the focus of our work, we only consider input-output examples as oracles
% - TODO: emphasize on the fully-automated nature of our approach -- we don't require test cases, and that is a differentiator from prior APR work
% - TODO: in our study we consider techniques prompt length

\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.5]
    {figures/overview.pdf}
    \caption{Code generation in the presence of an oracle overview. \bpaulse{fallback methods also can leverage the generated code and  task itself}}
    \label{fig:overview}
\end{figure}

In this work, we bridge this gap by performing a comprehensive study of fallback methods.
%
We first develop a categorization of fallback methods.
%
A fallback method can (1) \textit{restart} wherein the code candidate is thrown away and a new one is generated with a new query, (2) \textit{repair} wherein we attempt to repair the code candidate using the counterexample, (3) \textit{respond} wherein a back-and-forth dialogue is built up with the LLM, and (4) \textit{parameter search} wherein model parameters, e.g. temperature, are tuned.
%
Prior work has only considered techniques in (3) \textit{respond}, which is unfortunate since the dialogue can become impractically large for real-world code.
%
We propose a total of seven techniques, five of which have not been considered in prior work.



We scope our study of fallback methods to those that require little effort to adapt to new languages. 
%
To the best of our knowledge, only LLMs fall into this category.
%
A comparison of LLM-based fallback methods is highly valuable for code generation tasks involving new languages like Rust, which lack a mature ecosystem of research tools, such as those for APR.
%
Traditional APR tools are out-of-scope because their implementations have the disadvantage of being tied to a specific language, like Java or Python \bpaulse{$\gets$ cite specific tools to back up claim that tools are tied to specific language, or get rid of this sentence}.
%
We also only consider fallback methods that leverage the same LLM used for code generation, and the LLM is leveraged \textit{as-is}, i.e. without re-training/fine-tuning.
%
Concretely, this means we limit our study to techniques that work with prompts and model hyperparameters (e.g. temperature).



Then to evaluate our fallback methods, we perform a case study of translating code to the Rust language.
%
We develop a code translation pipeline that leverages an LLM to generate a candidate translation, and a cross-language differential fuzzer which serves as an oracle \hfeniser{to check input output equivalence of translation}.
%
We solve several practical challenges in differential cross-language fuzzing, such as as converting data structures from one programming language to another, and comparing execution results between programs in two different languages.
%
We evaluate our code translation pipeline and fallback methods on a set of code translation benchmarks mined from \textit{real-world} open source projects.
%
To mine the benchmarks, we develop a tool which analyzes a code-base's call graph to discover sub-modules (\hfeniser{suggestion: sub-programs}), and then extracts it into a standalone, compilable sub-module.


To the best of our knowledge, our work is the first to develop and evaluate an oracle guided code translation pipeline.
%
All prior work in code translation either does not consider the presence of an oracle, or assumes that test cases are available.
%
This assumption limits the practical usefulness of prior work.
%
In addition, this is the first work in code translation to evaluate on a large corpus of benchmarks extracted from real-world code.
%
While very recent work considers real-world code, they only consider two relatively small libraries both for parsing command-line arguments.\todo{cite}
%
Our work on the other hand considers a wide variety of libraries.


We evaluate our code translation pipeline and fallback methods on XX benchmarks in C and Go, resulting in a total of XX code translation experiments.
%
Our experimental results show that... \bpaulse{TODO: summarize results}


Contributions:
\begin{itemize}
    % We are not the first to do this anymore. There is an ICSE 2024 paper
    % \item We are the first to study LLM-based transpilation in real world code.
    \item We develop two oracles for determining a successful transpilation.
    \item We present a portfolio of fallback methods for managing failed transpilations and conduct a comprehensive evaluation process. 
    \item We introduce novel instantiations of the fallback methods.
    \item We open-source our implementation and the benchmarks which consists of more than 500 C and Go programs and their test corpora to accommodate further advances in code translation field. 
\end{itemize}



==> old/intro2.tex <==
\section{Introduction}
\label{section:intro}


% motivate the use LLMs in code translation
% Recent work~\cite{} has shown that large, generalist language models (simply ``LLMs'' in this work), such as ChatGPT, are highly effective for program transpilation -- the task of translating a program from a source language to a different target language. 
%
% They are particular well-suited to the task because they work out-of-the-box on most programming languages without fine-tuning. Moreover, they are highly adaptable. For example, they can learn to use new tools and libraries by pasting documentation directly into the prompt~\cite{zeroshottoolusage}.
%
% However, LLMs still may generate incorrect translations that do not faithfully preserve the behavior of the original source program, and due to the stochastic techniques employed in LLM inference, this issue is unlikely to ever be resolved.

Program transpilation is concerned with translating  source code written in one language to another language, with a similar level of abstraction. This task is becoming particularly relevant, given the recent interest in new, safe programming languages such as Rust, and, the expectation of translating potentially buggy, legacy code into such modern languages~\cite{c2rust,zhang2022repairing}. At the same time, the promise of large, generalist language models (simply “LLMs” in this work) like ChatGPT, provides the hope that transpilation can be done automatically by the LLMs. However, a recent study suggests that LLMs struggle to produce correct translations~\cite{PanICSE24}. 


% In this work, we study how an \textit{oracle} can be leveraged in LLM-driven code translation.
% Despite the fact that the original source program can serve as an oracle to validate the translation against, no work in LLM-driven code translation has studied how it could be leveraged. 
% In this work, we address  is to leverage the original source program as an \textit{input-output oracle} that provides the correct input for a given output.
% Fortunately, the original source program can be leveraged as an \textit{input-output oracle} that provides the correct input for a given output.

% introduce the idea of using an oracle in translation
In code transpilation, the original source program can serve as an \textit{input-output oracle} that provides the correct output for a given input.
%
It is straightforward to use such an oracle in order to validate the correctness of the translation: if, provided with the same inputs, the source program and the candidate translation produce the same outputs, then the candidate translation is said to preserve the semantics of the source program, which is the desired behaviour.

However, it is less clear how to proceed if the oracle finds distinguishing inputs, i.e. inputs for which the source program and the candidate translation produce different outputs. The recent study suggests incorporating additional information about the failure (e.g. failing tests) in the LLM query~\cite{PanICSE24}. In this work, we challenge this belief, and conduct a systematic investigation of the types of feedback that can be provided to the LLM and their respective efficacy.
%
% By comparing the outputs of the original source program and the candidate translation produced by the LLM on the same input, we can validate the correctness of the translation, or discover counterexample where they differ.
%
% However, there are several challenges to address to practically leverage the oracle.

% motivate the study of llm-based code generation with input-output oracles
% In code transpilation, the source implementation can serve as an \textit{input-output oracle} that provides the correct output for a given input. Despite their state-of-the-art performance at transpilation, LLMs still generate code that has different behavior from this oracle, and existing work in code transpilation does not make use of the oracle for correctness. 

% introduce the problem of correcting mistakes, define "fallback method", and go over the flow of the figure
In our work, we investigate the following question: when a counterexample is discovered, what techniques are effective for providing feedback to the LLM to fix it?
%
We refer to these techniques as \textit{fallback methods}.
To the best of our knowledge, this work is the first to develop and evaluate an LLM-based code transpilation pipeline that systematically investigates oracle-guided fallback strategies.
%
Figure~\ref{fig:overview} illustrates at a high-level what a  fallback method does, and how they are used in code transpilation.
% \todo{In this version we'll need to redo the figure slightly}
%
As shown in the figure, a description of a code transpilation task is first given to an LLM, which generates a code candidate. 
%
We then check the correctness of the candidate by comparing it with the original source program.
%
In our work, we develop a cross-language differential fuzzer to search for inputs where the original program and candidate produce different outputs.
% We use a cross-language fuzzer to check the behavior of the code candidate against the oracle. The fuzzer may provide a counterexample containing a program input, the expected output of the oracle, and the actual output of the code candidate.
%
If a counterexample is found, we apply a fallback method. A fallback method uses passing and failing tests, the candidate code, and the original query to construct a new query to the LLM 
%{\color{blue} Is it the case that a new query is always constructed? How about for parameter search? An alternative could be: If a counterexample is found, we apply a fallback method, which decides on the appropriate feedback to provide back to the LLM.} \bpaulse{Yes, a new query is always made to the LLM. In parameter search, there is still a new query}
%\cd{I don't think that's the case for simplification. If we go with the suggested alternative, we can reconcile alg 1 and alg 2 (not necessarily in an elegant manner, but still..).}.
%
A new code candidate is generated with the new query, and this process repeats until no counterexamples are returned.

To answer the above question, we first develop a categorization of fallback methods.
%
A fallback method can
\begin{enumerate}
    \item \textit{restart} by throwing away the code candidate is thrown away and generating a new query,
    \item \textit{repair} by attempting to repair the code candidate using the counterexample, or additional information obtained from the LLM itself,
    \item \textit{partition} by breaking up large tasks into smaller sub-problems,
%\textit{respond} by building a back-and-forth dialogue with the LLM, and
    \item \textit{parameter search} by automatically tuning model parameters, e.g. temperature.
\end{enumerate}
%
% Prior work has only considered techniques in 3) \textit{respond}, which quickly hits scalability limits as the dialogue can become impractically large for real-world code.
%
We propose a total of seven fallback techniques across these categories.


We then determine which strategies of fallback methods are the most effective by performing a case study of translating Go and C code to the Rust language.
%
We choose these languages because Go, C, and Rust are typically used for low-level programming tasks, such as systems development, and because of the recent interest in translation to Rust~\cite{c2rustpapers}.
%
% Unlike prior work, we emphasize heavily on translation benchmarks taken from real-world code.
We develop a code translation pipeline that uses an LLM to generate a candidate translation, and a cross-language differential fuzzer to query the oracle.
%
We evaluate our code translation pipeline and fallback methods on code translation benchmarks mined from \textit{real-world} open source projects.
%
% We develop a tool to mine the benchmarks. The tool analyzes a code base's call graph to discover sub-modules, and then extracts each into a standalone, compilable sub-module.

% brandon: I think our C benchmarks don't make too much use of memory management
% We picked  C and Go as source languages due to their different memory management protocols, with the former being manually managed, and the latter using a garbage collector. Memory management plays a central role in Rust, and finding the correct mapping between source and target is particularly difficult, even when done manually by experienced programmers. Considering different memory management protocols for the source language increases the confidence in the results of the study, as well as their transferability to other languages.

Our differential fuzzer is of capable comparing programs in C or Go to a candidate Rust translation, and it supports programs using complex data types (e.g. structs or classes) with pointers and any primitive types.
%
We solve the problem of executing a non-Rust program from Rust by using foreign function interfaces, enabling us to gather coverage information about both the original program and the translation during fuzzing. 
%
Since our fuzzer generates inputs using Rust data types, we solve the problem of passing this data to the original source program using serialization libraries common to nearly all programming languages.
%
We leverage this same solution for comparing outputs between the original program and the Rust translation.


Our work is the first comprehensive study of such fallback methods.
%
Most prior work in code generation tasks using LLMs~\cite{singlegencodegenworks,progsynthwLLMs,singlegenerationAPRworks,singlegenerationCodeTranslationworks} do not use counterexamples to improve their results.
%
Only very recent works have considered the presence of an tests ~\cite{APRandTranslationworks}, however the fallback methods they only consider two of the seven techniques considered in this work.
%
Specifically, they either repeat the same query to get a new code candidate, or they provide the failing input and the correct output as a response to the LLM and ask the LLM to fix it.


Our work is also the first to develop and evaluate an oracle guided code translation pipeline.
%
All prior work in code translation either does not consider the presence of an oracle, or assumes that test cases are available before transpilation.
%
This is also the first work in code translation to evaluate on a large corpus of benchmarks extracted from real-world code.
%
While very recent work considers real-world code, they only consider two relatively small libraries both for parsing command-line arguments.\todo{cite}





% Fallback methods are useful for LLM code generation tasks beyond code transpilation. They only need the original generation prompt and output, along with sets of failing and (optionally) passing tests. These tests could be produced by fuzzers, existing test suites, or program verification/validation tasks. 


% - TODO: mention program synthesis from examples and/or specifications
% - TODO: clarify that compilers as oracles is not the focus of our work, we only consider input-output examples as oracles
% - TODO: emphasize on the fully-automated nature of our approach -- we don't require test cases, and that is a differentiator from prior APR work
% - TODO: in our study we consider techniques prompt length

\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.5,clip,trim=3.8cm 8.9cm 14cm 2.5cm]{figures/overview.pdf}
    \caption{Code generation in the presence of an oracle overview. \bpaulse{fallback methods also can leverage the generated code and  task itself}}
    \label{fig:overview}
\end{figure}


We scope our study of fallback methods to those that require little effort to adapt to new languages. 
%
To the best of our knowledge, only LLMs fall into this category.
%
Scoping our work in this way makes it valuable for code generation tasks involving new languages like Rust, which lack a mature ecosystem of research tools, such as those for APR.
%
To manage cost and complexity we also only consider fallback methods that use the same LLM used for code generation \textit{as-is}, i.e. without re-training or fine-tuning.
%
Concretely, this means our study only modifies prompts and model hyperparameters (e.g. temperature).


We evaluate our code translation pipeline and fallback methods on XX benchmarks in C and Go, resulting in a total of XX code translation experiments.
%
Our experimental results show that... \bpaulse{TODO: summarize results}


Contributions:
\begin{itemize}
    \item we build a cross-language fuzzer, allowing us to query an oracle for transpilation, 
    \item we present a portfolio of fallback methods for managing failed transpilations and conduct a comprehensive evaluation process, and
    \item we open-source our implementation and the benchmarks which consists of more than 500 C and Go programs and their test corpora to accommodate further advances in code translation field. 
\end{itemize}

==> old/intro3.tex <==
\section{Introduction}
\label{section:intro}

\cd{
Program transpilation is concerned with translating  source code written in one language to another language, with a similar level of abstraction. This task is becoming particularly relevant, given the recent interest in new, safe programming languages such as Rust, and, the expectation of translating potentially buggy, legacy code into such modern languages.

At the same time, the promise of large, generalist language models (simply “LLMs” in this work), such as ChatGPT, provides the hope that transpilation can be done automatically by the LLMs. Unfortunately, a recent work casts doubt on this belief.  In particular, the robust study conducted in \cite{PanICSE24} revealed that LLMs can't be reliably used to automate code translation, with correct translations ranging from 2.1\% to 47.3\% for the studied LLMs. Even worse, the study concluded that the LLMs were largely ineffective on real-world projects, with success rates of 8.1\% for GPT-4 and 0\% for the rest of the models. As a 
way of improving the performance of the LLMs, the authors of \cite{PanICSE24} propose an iterative prompting approach that incorporates additional information about the failure (e.g. previous unsuccessful translation, stack trace, error messages from failing execution, failing test cases), which they found it increases the success rate by 5.5\%, on average.

In the current work, we revisit and challenge some of the conclusions of this recent study. In particular, our focus is on investigating the efficacy of a number of fallback strategies applied whenever the LLM provides an incorrect answer to a translation task:
\begin{enumerate}
    \item restart by throwing away the code candidate and generating a new query,
    \item repair by providing information about the error the code candidate using the counterexample,
    \item respond by building a back-and-forth dialogue with the LLM, and
    \item parameter search by automatically tuning model parameters, e.g. temperature.
\end{enumerate}

Our conclusion is that the conventional wisdom (perpetuated by \cite{PanICSE24} ) that providing more information to the LLM might not hold true for translation tasks. Instead, we showcase the advantage of other fallback/recovery techniques, such as restarts. \textbf{[here we need some numbers]}

The particular transpilation problem we address in this paper is that of going from C and Go to Rust. We picked  C and Go as source languages due to their different memory management protocols, with the former being manually managed, and the latter using a garbage collector. Memory management plays a central role in Rust, and finding the correct mapping between source and target is particularly difficult, even when done manually by experienced programmers. Considering different memory management protocols for the source language increases the confidence in the results of the study, as well as their transferability to other languages.

In order to make the problem more challenging, and avoid contaminating the study's results, we exclude the handling of Rust compilation errors from the study. The reason for this decision is the fact that the Rust compiler provides comprehensive error messages (containing clear suggestions for fixing the errors), which result in a much higher repair rate for the LLM than for other errors. (We handle these errors separately with a success rate of ...\%).

We are considering real-world benchmarks.
}


Program transpilation is concerned with translating  source code written in one language to another language, with a similar level of abstraction. This task is becoming particularly relevant, given the recent interest in new, safe programming languages such as Rust, and, the expectation of translating potentially buggy, legacy code into such modern languages. At the same time, the promise of large, generalist language models (simply “LLMs” in this work) like ChatGPT, provides the hope that transpilation can be done automatically by the LLMs. However, a recent study suggests that LLMs struggle to produce correct translations~\cite{PanICSE24}. 
% They also experiment with an iterative repair approach to fix incorrect translations, though with limited success, and suggest that providing additional context to the LLM may yield better results.

% In this work, we study how an \textit{oracle} can be leveraged in LLM-driven code translation.
% Despite the fact that the original source program can serve as an oracle to validate the translation against, no work in LLM-driven code translation has studied how it could be leveraged. 
% In this work, we address  is to leverage the original source program as an \textit{input-output oracle} that provides the correct input for a given output.
% Fortunately, the original source program can be leveraged as an \textit{input-output oracle} that provides the correct input for a given output.

% introduce the idea of using an oracle in translation
During code transpilation, the original source program can serve as an \textit{input-output oracle} that provides the correct output for a given input.
%
It is straightforward to use such an oracle to validate the correctness of the translation: if, provided with the same inputs, the source program and the candidate translation produce the same outputs, then the candidate translation is said to preserve the semantics of the source program, which is the desired behaviour.

However, it is less clear how to proceed if the oracle finds distinguishing inputs, i.e. inputs for which the source program and the candidate translation produce different outputs. The recent study~\cite{PanICSE24} suggests incorporating additional information about the failure (e.g. failing tests) in the LLM query. In this work, we challenge this belief, and conduct a systematic investigation of the types of feedback that can be provided to the LLM and their respective efficacy.

% By comparing the outputs of the original source program and the candidate translation produced by the LLM on the same input, we can validate the correctness of the translation, or discover counterexample where they differ.
%
% However, there are several challenges to address to practically leverage the oracle.

% motivate the study of llm-based code generation with input-output oracles
% In code transpilation, the source implementation can serve as an \textit{input-output oracle} that provides the correct output for a given input. Despite their state-of-the-art performance at transpilation, LLMs still generate code that has different behavior from this oracle, and existing work in code transpilation does not make use of the oracle for correctness. 

% introduce the problem of correcting mistakes, define "fallback method", and go over the flow of the figure
The following question remains unanswered in the literature: what techniques are effective in providing feedback to the LLM to correct buggy translations?
%
We refer to these techniques as \textit{fallback methods}.
%
% To the best of our knowledge, this work is the first to develop and evaluate an LLM-based code transpilation pipeline that systematically investigates oracle-guided fallback strategies.
%
Figure~\ref{fig:overview} illustrates at a high-level how fallback methods fit into the code translation process.
% what a fallback method does, and how they are used in code transpilation. \todo{In this version we'll need to redo the figure slightly}
%
As shown in the figure, a description of a code translation task is first given to an LLM, which generates a candidate translation. 
%
The correctness of the translation is then checked against an \textit{oracle}.
%
The oracle takes the translation, and returns a set of counterexamples where the translation's output differs from the original source program.
%
% We then check the correctness of the candidate by comparing it with the original source program.
%
% In our work, we develop a cross-language differential fuzzer to search for inputs where the original program and candidate produce different outputs.
% We use a cross-language fuzzer to check the behavior of the code candidate against the oracle. The fuzzer may provide a counterexample containing a program input, the expected output of the oracle, and the actual output of the code candidate.
%
If a counterexample is returned, we apply a fallback method. A fallback method uses passing and failing tests, the candidate code, and the original query to construct a new query to the LLM.
% {\color{blue} Is it the case that a new query is always constructed? How about for parameter search? An alternative could be: If a counterexample is found, we apply a fallback method, which decides on the appropriate feedback to provide back to the LLM.}
%
A new code candidate is generated with the new query, and this process repeats until no counterexamples are returned.

In our work, the oracle 

To answer the above question, we first develop a categorization of fallback methods.
%
A fallback method can
\begin{enumerate}
    \item \textit{restart} by throwing away the code candidate is thrown away and generating a new query,
    \item \textit{repair} by attempting to repair the code candidate using the counterexample,
    \item \textit{respond} by building a back-and-forth dialogue with the LLM, and
    \item \textit{parameter search} by automatically tuning model parameters, e.g. temperature.
\end{enumerate}
%
% Prior work has only considered techniques in 3) \textit{respond}, which quickly hits scalability limits as the dialogue can become impractically large for real-world code.
%
We propose a total of seven fallback techniques across these categories.


We then determine which strategies of fallback methods are the most effective by performing a case study of translating code to the Rust language.
%
We develop a code translation pipeline that uses an LLM to generate a candidate translation, and a cross-language differential fuzzer to query the oracle.
%
We evaluate our code translation pipeline and fallback methods on code translation benchmarks mined from \textit{real-world} open source projects.
%
We develop a tool to mine the benchmarks. The tool analyzes a code base's call graph to discover sub-modules, and then extracts each into a standalone, compilable sub-module.



Our differential fuzzer is of capable comparing programs in C or Go to a candidate Rust translation, and it supports programs using complex data types (e.g. structs or classes) with pointers and any primitive types.
%
%
We solve the problem of executing a non-Rust program from Rust by using foreign function interfaces, enabling us to gather coverage information about both the original program and the translation during fuzzing. 
%
Since our fuzzer generates inputs using Rust data types, we solve the problem of passing this data to the original source program using serialization libraries common to nearly all programming languages.
%
We leverage this same solution for comparing outputs between the original program and the Rust translation.


Our work is the first comprehensive study of such fallback methods.
%
Most prior work in code generation tasks using LLMs~\cite{singlegencodegenworks,progsynthwLLMs,singlegenerationAPRworks,singlegenerationCodeTranslationworks} do not use counterexamples to improve their results.
%
Only very recent works have considered the presence of an tests ~\cite{APRandTranslationworks}, however the fallback methods they only consider two of the seven techniques considered in this work.
%
Specifically, they either repeat the same query to get a new code candidate, or they provide the failing input and the correct output as a response to the LLM and ask the LLM to fix it.


Our work is also the first to develop and evaluate an oracle guided code translation pipeline.
%
All prior work in code translation either does not consider the presence of an oracle, or assumes that test cases are available before transpilation.
%
This is also the first work in code translation to evaluate on a large corpus of benchmarks extracted from real-world code.
%
While very recent work considers real-world code, they only consider two relatively small libraries both for parsing command-line arguments.\todo{cite}





% Fallback methods are useful for LLM code generation tasks beyond code transpilation. They only need the original generation prompt and output, along with sets of failing and (optionally) passing tests. These tests could be produced by fuzzers, existing test suites, or program verification/validation tasks. 


% - TODO: mention program synthesis from examples and/or specifications
% - TODO: clarify that compilers as oracles is not the focus of our work, we only consider input-output examples as oracles
% - TODO: emphasize on the fully-automated nature of our approach -- we don't require test cases, and that is a differentiator from prior APR work
% - TODO: in our study we consider techniques prompt length

\begin{figure}[t!]
    \centering
    \includegraphics[scale=0.5,clip,trim=3.8cm 8.9cm 14cm 2.5cm]{figures/overview.pdf}
    \caption{Code generation in the presence of an oracle overview. \bpaulse{fallback methods also can leverage the generated code and  task itself}}
    \label{fig:overview}
\end{figure}


We scope our study of fallback methods to those that require little effort to adapt to new languages. 
%
To the best of our knowledge, only LLMs fall into this category.
%
Scoping our work in this way makes it valuable for code generation tasks involving new languages like Rust, which lack a mature ecosystem of research tools, such as those for APR.
%
To manage cost and complexity we also only consider fallback methods that use the same LLM used for code generation \textit{as-is}, i.e. without re-training or fine-tuning.
%
Concretely, this means our study only modifies prompts and model hyperparameters (e.g. temperature).


We evaluate our code translation pipeline and fallback methods on XX benchmarks in C and Go, resulting in a total of XX code translation experiments.
%
Our experimental results show that... \bpaulse{TODO: summarize results}


Contributions:
\begin{itemize}
    \item we build a cross-language fuzzer, allowing us to query an oracle for transpilation, 
    \item we present a portfolio of fallback methods for managing failed transpilations and conduct a comprehensive evaluation process, and
    \item we open-source our implementation and the benchmarks which consists of more than 500 C and Go programs and their test corpora to accommodate further advances in code translation field. 
\end{itemize}



==> old/intro4.tex <==
\section{Introduction}
\label{section:intro}
Program transpilation, the task of translating one programming language to another, has many practical uses such as translating legacy code to modern languages~\cite{RoziereLachaux2020,C2Rust}. While language-specific transpilation tools have been developed~\cite{C2Rust,zhang2022heterogen,emre2021translating},
large language models (LLMs) provide hope that this task can be done automatically~\cite{szafraniec2022code,RoziereLachaux2020,RoziereZhang2022,mariano2022automated}. Unfortunately however, recent work shows that current LLMs cannot reliably translate code~\cite{PanICSE24}. Their study reports a successful translation rate of just 8\% on a small sample of real-world code. 
% The authors experiment with an iterative feedback strategy, however they show an improvement in success rate of only 12\% at most, and do not consider other techniques.

To address this issue, we propose and evaluate a diverse set of feedback strategies that increase the transpilation success rate on real-world code by 17.5\% on average, leading to an absolute increase in average overall success rate from 23.3\% to 40.7\%. \todo{Update numbers.}
%
We achieve these improvements without using a significant amount of the available prompt window. 
%
We show a different path than the conventional wisdom (perpetuated by \cite{PanICSE24}) that providing more information to the LLM is the path forward.


Our feedback strategies may not be surprising to anyone who has corrected mistakes made by students. Rather than asking them to read a textbook, a teacher might:
\begin{enumerate}
    \item simply ask them to try again,
    \item call out a mistake, and ask them to try again,
    % It's really hard to differentiate between the above item and the below item
    % \item have a conversation about the mistake, and work with them to build a new solution,
    \item work with them to break the problem into sub-problems,
    \item suggest that they try a more (or less) creative solution.
\end{enumerate}
Our feedback strategies follow these exact lines of reasoning, resulting in concise prompts with a high chance of success. 


Figure~\ref{fig:overview} illustrates the flow of feedback strategies. As shown in the figure, a description of a code-translation task is first given to an LLM, which generates a candidate translation. 
%
The correctness of the translation is then checked against an \textit{oracle}.
%
The oracle takes the translation and returns a set of counterexamples, i.e., inputs for which the translation's output differs from the original source program.
% We then check the correctness of the candidate using an \textit{oracle routine}. 
Many of our feedback strategies make use of counterexamples.
%
In particular, if the translation was incorrect, we create a new prompt using any previous dialogue with the LLM, the incorrect translation, and counterexamples returned by the oracle. 
%
We repeat this process iteratively, until some fixed number of iterations is reached or the translation is deemed correct by the oracle. 

% We evaluate our strategies on a translation into to Rust. We use both C and Go as source languages due to their different memory management protocols, with the former being manually managed, and the latter using a garbage collector. Memory management plays a central role in Rust, so finding the correct mapping between source and target is particularly difficult, even when done manually by experienced programmers. Considering different memory management protocols for the source language increases the confidence in the results of the study, as well as their transferability to other languages.

We design our oracle such that it is capable of automatically discovering counterexamples between the candidate translation and the original source program.
This allows our approach to work with code that does not already have unit tests.
%
The oracle takes as input the original program and its translation and performs cross-language differential fuzzing to discover inputs where they differ in output.
% To implement the oracle routine, 
% we develop a cross-language differential fuzzer to check the correctness of the translation and generate counterexamples. 
It supports programs using complex data types (e.g., structs or classes), pointers, and any primitive types. 
%
We drive the fuzzing search with coverage information about both programs.


We combine our oracle, feedback strategies, and LLM into an end-to-end, automated code-translation tool and evaluate it on translation benchmarks mined from real-world, open-source projects.
%
This represents a significant step forward in assessing the practicality of code translation.
%
% We evaluate our code translation pipeline and prompt refine on code translation benchmarks mined from \textit{real-world} open source projects.
%
We develop a methodology and tool to automatically mine benchmarks.
%
Our mining tool takes as input a whole project and a specific function in the project.
%
It then extracts the given function and all of its dependencies, including that function's callees, structs, global variables, etc., into a single, compilable file, which we use directly as the benchmark.
%
This enables us to automatically gather a large number of benchmarks  from real-world code.

Our work is the first comprehensive study of feedback strategies for LLM-based code transpilation, and even code generation in general.
%
Most prior work on code-generation tasks using LLMs (including transpilation)~\cite{zhang2023multilingual,tang-etal-2023-explain,yan2023codetransocean,jana2023attention,mariano2022automated,szafraniec2022code,poesia2022synchromesh,nijkamp2022codegen,austin2021program,ni2023lever,gou2023critic,chen2023teaching,madaan2023selfrefine,zhang2022repairing,peng2024domain,joshi2023repair} does not consider the presence of an oracle when generating code, and thus, it does not consider feedback strategies. 
%
Test cases are only executed after the final code is generated to measure accuracy, and there is no attempt to fix incorrect code.
%
Only very recent work has considered the presence of tests, which can serve as an oracle, during code generation~\cite{PanICSE24,xia2023conversational,xia2023automated,xia2022less}. However, the feedback strategies they consider are limited, and no insights are provided into which strategies perform better.
%
% Specifically, they either repeat the same query to get a new code candidate, or they provide the failing input and the correct output as a response to the LLM and ask the LLM to fix it.
% This is also the first work in code translation to evaluate on a large corpus of benchmarks extracted from real-world code.
%

In addition, our work is the first to study the effectiveness of LLM-based code translation on a large and diverse set of benchmarks extracted from real-world code.
%
While very recent work in code translation considers real-world code~\cite{PanICSE24}, their study was limited to 37 benchmarks taken from a single application domain.
%
In contrast, we evaluate our approach on over 300 benchmarks taken from four different application domains.


% - TODO: mention program synthesis from examples and/or specifications
% - TODO: emphasize on the fully-automated nature of our approach -- we don't require test cases, and that is a differentiator from prior APR work
% - TODO: in our study we consider techniques prompt length

\begin{figure}[t!]
    \centering
    % \includegraphics[scale=0.7,trim=6cm 14cm 5cm 7cm]
    \includegraphics[scale=0.45]
    {figures/overview2.pdf}
    \caption{Code translation using feedback strategies.}
    \label{fig:overview}
\end{figure}

% We scope our study of refinement strategies to those that use only an LLM, the 
% %
% To the best of our knowledge, only LLMs fall into this category.
% %
% Scoping our work in this way makes it valuable for code generation tasks involving new languages like Rust, which lack a mature ecosystem of research tools, such as those for APR.
% %
% To manage cost and complexity we also only consider fallback methods that use the same LLM used for code generation \textit{as-is}, i.e. without re-training or fine-tuning.
% %
% Concretely, this means our study only modifies prompts and model hyperparameters (e.g. temperature).


Because our goal is to improve the use of LLMs for code transpilation, we only consider feedback strategies that leverage the LLM and the counterexamples returned by the oracle.
%
More traditional, non-LLM based techniques, such as those for automated program repair, are out-of-scope for our study, though we note that recent work shows LLMs are fair well compared to these techniques.
%
Scoping our work in this way makes it valuable for code generation tasks involving new languages like Rust, which lack a mature ecosystem of research tools, such as those for APR.

We evaluate the effectiveness of our strategies on the task of translating Go and C code to Rust.
%
We choose these languages because Go, C, and Rust are typically used for low-level programming tasks, such as system development, and because of the recent interest in translating to Rust~\cite{C2Rust,ling2022rust,zhang2023ownership,emre2021translating}.
In total, we evaluate our translation pipeline using a state-of-the-art LLM, Claude 2~\cite{claude}, and seven different feedback strategies on a set of almost 307 C and Go translation benchmarks mined from four open source projects on GitHub.
In total, we report results 2,149 code translation experiments.
%
Our experimental results lead to several key insights.
%
First, our feedback strategies can increase the success rate by up to 17.5\% on average, leading to an overall average success rate of 40.7\%. This represent a significant step up from the 8\% reported in prior work~\cite{PanICSE24}.
%
Second, we find that our partitioning feedback method, which breaks a translation task into sub-tasks, often has the best performance overall.
%
And third, we find that providing counterexamples in the initial translation task description yields almost the same improvement as providing the counterexamples as a response to the LLM, suggesting an approach to significantly reduce prompt size.

In summary, we make the following contributions:
\begin{itemize}
    \item We present a diverse set of feedback strategies that are applicable to code translation with LLMs 
    \item We implement our feedback strategies in an end-to-end translation tool for Rust
    \item We evaluate our translation tool on a diverse set of C and Go benchmarks mined from real-world code, which shows our feedback strategies yield 17.5\% improvement in translation success rates, and an 40.7\% overall success rate
    \item We open-source all of our code, benchmarks, and results
    % which consists of more than 500 C and Go programs and their test corpora to accommodate further advances in code translation field. 
\end{itemize}

==> partition.tex <==
\paragraph{Task Partitioning \partition } Another option when a task is too difficult for the LLM is to break it into smaller subtasks. In the context of the current translation problem, this amounts to splitting the source program into smaller chunks, as illustrated by Alg. \ref{alg:simplification}. In particular, we start by translating the include statements, structs and global variables. In Alg. \ref{alg:simplification}, these are part of the header $h$. Method \textsc{prompt} constructs the required prompt as described in Fig.\ref{figure:translate-prompt}. This is subsequently used to invoke the LLM at line 2. We use  map $T$ to store all the translated code.

After translating the header, we perform a post-order traversal of the call graph, translating each function as we visit it. Assuming the absence of recursion, this ensures that a function's dependencies have already been translated before we translate that function. We handle recursion by translating sets of functions that form a cycle in the call graph together.

% which we traverse in post-order so that the leaves (i.e. functions that do not call any other functions) are translated first. Once those are translated, we proceed to their parents in the call graph, essentially always translating functions whose callees were already translated. 
The algorithm is shown in Alg.~\ref{alg:simplification}. For each function $f$
to translate, we construct the prompt using the function's code, the translated header, $T(h)$, and the already translated code for the function's callees, $T(\textsc{callees}(f))$ (line 5).  If we reached the entry point of program $p$ (which corresponds to the root of the call graph), then, at line 7, we return the prompt. This will be used in Alg. \ref{alg:genworacle} to obtain the final translation, i.e. the translation of the whole program, which will subsequently be checked by the oracle. If we didn't reach the entry point, then, at line 9, we invoke the LLM using the most recent prompt, and store the translation for $f$. 
%
\Cref{fig:simplify-prompt} illustrates an example of how the prompt is constructed during task partitioning: the first prompt is used to translate the header; then, the second prompt is intended to translate ``Function 1'', while using the previous translation of the header; following the same pattern, the third prompt aims to translate ``Function 2'', and relies on the previous translations for header and ``Function 1''. 
%At line 8, we return the concatenation of all the translations stored in map $T$, essentially corresponding to the translation for program $p$. 
For ease of presentation, Alg.\ref{alg:simplification} doesn't capture the treatment of mutually recursive functions, which are translated at the same time (i.e. with the same prompt).

\begin{algorithm}
\caption{Task Partitioning}
\label{alg:simplification}
\begin{algorithmic}[1]
  \Require $p$ : Program to translate
  \State $h \gets \textsc{header}(p)$
  \State $T(h)\gets G(\textsc{prompt}(h))$
  \State $g \gets \textsc{call}{-}\textsc{graph}(p)$
  \For{$f \in \textsc{post}{-}\textsc{order}(g)$}
  \State $q \gets \textsc{prompt}(f, T(h),T(\textsc{callees}(f)))$
        \If{$\textsc{entry-point}(f)$}
            \State \textbf{return} $q$
        \EndIf
        \State $T(f) \gets G(q)$
\EndFor
\State \textbf{return} $\textsc{FAIL}$
%\State \textbf{return} $T.\textsc{reduce}(+)$
\end{algorithmic}
\end{algorithm}


%\cd{For Alg 2, the oracle needs to be called on the full translation of program $p$. However, that's not yet in as it needs to be decided how to reconcile this alg with alg1.}

%\paragraph{Task Simplification (\simplify)} It is possible that the LLM is generating a program that fails oracle checks because the task is inherently too complex to be handled in a single iteration. In such cases, breaking down the original task into reasonably sized sub-tasks and querying the LLM for each of them separately could be a more effective approach. In \Cref{alg:simplify}, we introduce a novel task simplification method for code translation use-case. According to it, we start with decomposing (\Cref{line:decompose}) the given program into smaller chunks consisting of one function. Any program component outside of the functions such as include statements, structs or global variables are put in one chunk, \emph{header-chunk}. The chunks are topologically sorted based on the functions' order in the program call-graph and header-chunk is placed in the first position. The main idea is to obtain translation of one chunk at each iteration.
% Later, we iterate over the chunks get the  and 
%Prompt building, however, is more complicated; we construct each prompt by building upon the previous one (\Cref{line:simplify-prompt}). More specifically, at each iteration we add one new chunk to the prompt and keep the previous generations to reinforce the LLM's previous understanding. We continue this process until all pieces are translated. 
%\todo{how does this relate to CoT}
%\begin{algorithm}
%\caption{\simplify}
%\label{alg:simplify}
%\begin{algorithmic}[1]
  %\State $ dc \gets \mathsf{decompose}(c)$  \label{line:decompose}
  %\State $cur\_c$, $g \gets \mathsf{emptystr}$
  %\For{$d$ $\mathsf{in}$ $dc$}
    %\State $cur\_c \gets cur\_c + d$
    %\State $p \gets \mathsf{make\_prompt}(cur\_c, g)$ \label{line:simplify-prompt}
    %\State $ans \gets \mathsf{invoke\_llm(d)}$
    %\State $cur\_g \gets \mathsf{postprocess}(ans)$
    %\State $g \gets g + cur\_g$
  %\EndFor
  %\State \textbf{return} $g$
%\end{algorithmic}
%\end{algorithm}


%\Cref{fig:simplify-prompt} illustrates an example where the first prompt is built to obtain translation of the header-chunk. The second prompt keeps the header-chunk and appends the next chunk to it. Additionally, the answer to the previous prompt is kept in the current one. This way LLM is only asked to make a translation for the current chunk and is provided its previous translations for taking into consideration. The process ends when all pieces are translated.

\begin{figure}
    \centering
    \begin{tcolorbox}[
        colback=prompt_bg,
        colframe=prompt_title,
        title=Prompt Sequence for \simplify,
        subtitle style={boxrule=0.4pt, colback=yellow!50!blue!25!white, colupper=black},
    ]
    \scriptsize

    \tcbsubtitle{Prompt 1}
    \textbf{Human:}\\
    \textit{\# Code to be translated}\\
    \texttt{\{C Import/Struct statements, Global variables\}} \\
    
    \textit{\# Instruction and Constraints}\\
    \texttt{Translate above C program to Rust\dots}\\

    \textbf{Assistant:}\\

    \tcbsubtitle{Prompt 2}
    \textbf{Human:}\\
    \textit{\# Code to be translated}\\
    \texttt{\{C import/struct statements, global variables\}} \\
    \texttt{\{\textbf{C Function 1}\}} \\

    \textit{\# Instruction and Constraints}\\
    \texttt{Translate above C program to Rust\dots}\\

    \textbf{Assistant:}\\
    \texttt{\{Rust import/struct statements and global variables translated in previous step\}} \\
    
    \tcbsubtitle{Prompt 3}
    \textbf{Human:}\\
    \textit{\# Code to be translated}\\
    \texttt{\{C import/struct statements, global variables\}} \\
    \texttt{\{C Function 1\}} \\
    \texttt{\{\textbf{C Function 2}\}} \\

    \textit{\# Instruction and Constraints}\\
    \texttt{Translate above C program to Rust\dots}\\

    \textbf{Assistant:}\\
    \texttt{\{Rust import/struct statements and global variables translated in previous step\}} \\
    \texttt{\{Rust Function 1 translated in previous step\}} \\

    \tcbsubtitle{Prompt N}
    \dots
    \end{tcolorbox}
    \caption{LLM Prompt Sequence for \partition.}
    \label{fig:simplify-prompt}
\end{figure}

